MemPool: A Shared-L1 Memory Many-Core Cluster with a Low-Latency Interconnect

A key challenge in scaling shared-L1 multi-core clusters towards many-core (more than 16 cores) configurations is to ensure low-latency and efficient access to the L1 memory. In this work we demonstrate that it is possible to scale up the shared-L1 architecture: We present MemPool, a 32 bit many-core system with 256 fast RV32IMA "Snitch" cores featuring application-tunable execution units, running at 700 MHz in typical conditions (TT/0.80 V/25{\deg}C). MemPool is easy to program, with all the cores sharing a global view of a large L1 scratchpad memory pool, accessible within at most 5 cycles. In MemPool's physical-aware design, we emphasized the exploration, design, and optimization of the low-latency processor-to-L1-memory interconnect. We compare three candidate topologies, analyzing them in terms of latency, throughput, and back-end feasibility. The chosen topology keeps the average latency at fewer than 6 cycles, even for a heavy injected load of 0.33 request/core/cycle. We also propose a lightweight addressing scheme that maps each core private data to a memory bank accessible within one cycle, which leads to performance gains of up to 20% in real-world signal processing benchmarks. The addressing scheme is also highly efficient in terms of energy consumption since requests to local banks consume only half of the energy required to access remote banks. Our design achieves competitive performance with respect to an ideal, non-implementable full-crossbar baseline.

==> fig/benchmarks/result_bench_rel_arch <==
Kernels         Top1+S       Top1         Top4+S       Top4         TopH+S       TopH          TopX+S TopX
{\emph{matmul}} 0.2772409941 0.2385147247 0.7722464219 0.7149217071 0.8171193416 0.7455971822  1      1
{\emph{2dconv}} 0.7522974102 0.6919594528 0.7874945343 0.8089978138 0.882734959  0.8504898996  1      1
{\emph{dct}}    0.9865114298 0.4454638124 0.9716123619 0.8356639178 0.9856717265 0.8263798605  1      1


==> fig/benchmarks/result_bench_rel_arch_backup <==
Kernels         Top1+S       Top1         Top4+S       Top4         TopH+S       TopH          TopX+S TopX
{\emph{matmul}} 0.2736665736 0.2440460948 0.7622899813 0.7315013816 0.8065843621 0.7628882485  1      1
{\emph{2dconv}} 0.7769423559 0.7158744218 0.813292523  0.8369577724 0.9116529837 0.8798838757  1      1
{\emph{dct}}    1.047139003  0.4574413863 1.03132429   0.8581331421 1.046247695  0.8485994563  1      1


==> fig/benchmarks/result_bench_rel_best <==
Kernels         Top1+S       Top1         Top4+S       Top4         TopH+S       TopH         TopX+S       TopX
{\emph{matmul}} 0.2661267802 0.2440460948 0.7412881145 0.7315013816 0.7843621399 0.7628882485 0.9724489796 1
{\emph{2dconv}} 0.7596073517 0.7158744218 0.7951464801 0.8369577724 0.8913123392 0.8798838757 0.977688172  1
{\emph{dct}}    1.019451938  0.4574413863 1.004055377  0.8581331421 1.018584196  0.8485994563 0.973559322  1


==> fig/benchmarks/result_bench_runtime <==
Kernels         Top1+S Top1  Top4+S Top4 TopH+S TopH TopX+S TopX
{\emph{matmul}} 17905  19525 6428   6514 6075   6246 4900   4765
{\emph{2dconv}} 9576   10161 9148   8691 8161   8267 7440   7274
{\emph{dct}}    7043   15696 7151   8367 7049   8461 7375   7180

